Smoothed analysis of the low-rank approach for smooth semidefinite programs

We consider semidefinite programs (SDPs) of size n with equality constraints. In order to overcome scalability issues, Burer and Monteiro proposed a factorized approach based on optimizing over a matrix Y of size $n$ by $k$ such that $X = YY^*$ is the SDP variable. The advantages of such formulation are twofold: the dimension of the optimization variable is reduced and positive semidefiniteness is naturally enforced. However, the problem in Y is non-convex. In prior work, it has been shown that, when the constraints on the factorized variable regularly define a smooth manifold, provided k is large enough, for almost all cost matrices, all second-order stationary points (SOSPs) are optimal. Importantly, in practice, one can only compute points which approximately satisfy necessary optimality conditions, leading to the question: are such points also approximately optimal? To this end, and under similar assumptions, we use smoothed analysis to show that approximate SOSPs for a randomly perturbed objective function are approximate global optima, with k scaling like the square root of the number of constraints (up to log factors). Moreover, we bound the optimality gap at the approximate solution of the perturbed problem with respect to the original problem. We particularize our results to an SDP relaxation of phase retrieval.

==> RelatedWork.tex <==
\section{Related work}\label{PreviousWork}

Developing faster SDP solvers has drawn a fair amount of attention in both the optimization and the theoretical computer science communities. Most of the existing results for SDP solvers can be cast in two different approaches: direct, convex methods and factorization methods. We summarize previous work below.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A number of recent works aim to produce large-scale SDP solvers.
Among the direct approaches (which proceed in the convex domain directly), \citet{SPARSESDP} introduced a Frank-Wolfe type method for a restricted class of SDPs. Here, the key is that each iteration increases the rank of the solution only by one, so that if only a few iterations are required to reach satisfactory accuracy, then only low dimensional objects need to be manipulated. This line of work was later improved by \citet{HybridDSP}, \citet{FastSpecta} and \citet{SublinearSDP} through hybrid methods.
Still, if high accuracy solutions are desired, a large number of iterations will be required, eventually leading to large-rank iterates. In order to overcome such issue, \citet{SketchyDecisions} recently proposed to combine conditional gradient and sketching techniques in order to maintain a low rank representation of the iterates.


Among the low-rank approaches, our work is closest to (and indeed largely builds upon) recent results of~\citet{bhojanapalli2018smoothed}. For the real case, they consider a penalized version of problem~\eqref{eq:eq3} (which we here refer to as  (P-SDP)) and its related penalized Burer--Monteiro formulation, here called (P-P). With high probability upon random perturbation of the cost matrix, they show approximate global optimality of ASOSPs for (P-P), assuming $k$ grows with $\sqrt{m}$ and either the SDP is compact or its cost matrix is positive definite. 
Given that there is a zero-measure set of SDPs where SOSPs may be suboptimal, there can be a small-measure set of SDPs where ASOSPs are not approximately optimal~\citep{bhojanapalli2018smoothed}. In this context, the authors resort to smoothed analysis, in the same way that we do here.
%the idea is to perturb the cost matrix in order to obtain a perturbed SDP that is sufficiently far away from the pathological set with high probability. More specifically, if $Y\in \K^{n\times k}$ is an ASOSP of the perturbed version of (P-P) with $k=\tilde{\Omega}(\sqrt{m})$ and the residues $\left(\dotprod{A_i,X}-b_i\right)^2$ are bounded for $i=1,\dots,m$, then they establish that $X=YY^{*}$ is an approximate global  optimum of (P-SDP).
One important drawback of that work is that the final result does not hold for the original SDP, but for a non-equivalent penalized version of it. This is one of the points we improve here, by focusing on smooth SDPs as defined in~\citep{boumal2016non}.
% This paper corrects this flaw, by showing that in the case of smooth SDP and with high probability, any ASOSP for (P-P) is an approximate global optima for (P-SDP).
%\newline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection*{Convex methods}
%
% \hspace{\parindent}  The first polynomial algorithm for SDP was given by the ellipsoid method~\citep{Ellipsoid1}, ~\citep{Ellipsoid2}, ~\citep{Ellipsoid3}.
% Due to its poor empirical performances, interior point methods~\citep{PolyBarrier},~\citep{SelfBarrier},~\citep{IPM} and cutting-plane methods ~\citep{VolBarrier},~\citep{CuttingPlane}  allowing for an efficient implementation were later developed. 
%However ,in practice, the high computational cost of each iteration make those methods unadequate in the case of large scale instances.  Such caveat led to several research directions. 
% Restricting themselves to the class of SDPs with a trace constraint,~\citep{MWSDP} proposed a multiplicative weights based method. ~\citep{SPARSESDP} then introduced a Frank-Wolfe type method, which was later improved by ~\citep{HybridDSP}, ~\citep{FastSpecta}  and ~\citep{SublinearSDP} through hybrid methods.
%The fact that the rank of the solution of those methods increase with each iteration
%implies that those methods still suffer from a significant need for memory. In order to overcome such issue,~\citep{SketchyDecisions} proposed to combine conditional gradient and sketching techniques in order to maintain a low rank representation.
%
%\subsubsection*{Low-rank approaches}
%
%\hspace{\parindent} Burer and Monteiro were the first to study the factorized problem~\eqref{eq:eq4} for the purpose of solving~\eqref{eq:eq3}
%~\citep{burer2003nonlinear,burer2005local}. 
%~\cite{kulis2007fast} underlined the success of such low-rank approaches in practice: by considering the k-means clustering and the maximum variance unfolding problems, their approach is significantly faster, scalable and in some cases, produces better results compared to traditional SDP relaxation techniques.
%However, the non-convexity of the factorized problem raises questions about the optimality guarantees of this formulation. 
%Burer and Monteiro~\citep{burer2003nonlinear,burer2005local} first showed that any rank-deficient local optimum is optimal for the SDP.  
%This result was later extended to any rank-deficient SOSP for a restrictive class of SDP by~\citet{journee2010low}.
%The main issue is that none of those analyses guarantees that SOSPs are rank-deficient. 
%
%~\citet{boumal2016non} consider the setting 
%where Assumption~\ref{ass:smoothmanifold} holds and $\K=\R$. They show that for almost any symmetric cost matrix $C$, 
%if a matrix $Y\in \R^{n \times k}$ with $\frac{k(k+1)}{2} > m$
%is an SOSP of~\eqref{eq:eq4}, then $Y$ is globally optimal and $X=YY^{*}$ is globally 
%optimal for~\eqref{eq:eq3}. We stress that this statement excludes a zero-measure set of cost matrices. Therefore, for the SDPs associated to the 
%cost matrices in this set, there may exist suboptimal SOSPs. To obtain a similar result including all cost matrices, they require $k=n+1$, 
%which forfeits one of the initial reasons to use a factorization approach, namely, the dimensionality reduction. 
%Moreover, they provide optimality results for SOSPs only, while in practice only ASOSPs can be computed.
%In related work,~\cite{mei2017solving} 
%focus on the specific class of SDPs with elliptic constraints (including the Max-Cut SDP), for $\K=\R$. They show that 
%any rank-$k$ SOSP provides a $(1-\frac{1}{k-1})$--approximation to the optimal value of the problem. This result is interesting for its generality in $k$; in particular, 
%it readily provides some guarantees for $k=O(1).$ On the other hand, it does not accurately capture the approximate optimality of ASOSPs for large $k$, 
%and it holds for a class of SDP which is a subset of the ones covered here.
%
%
%
%\hspace{\parindent}To overcome some of the flaws mentioned above,~\cite{bhojanapalli2018smoothed} consider a penalized version (P-SDP) of problem~\eqref{eq:eq3} and its related 
%Burer-Monteiro formulation (P-P), when $\K=\R$. They show approximate global optimality of ASOSPs for (P-P), upon random
%perturbation of the cost matrix, with high probability, assuming $k$ grows with $\sqrt{m}$ and the SDP is either compact or 
%its cost matrix is positive definite. 
%Given that there is a zero-measure set of SDPs where SOSPs may be suboptimal, there can be a small-measure set of SDPs where ASOSPs
%are not approximately optimal~\citep{bhojanapalli2018smoothed}. In this context, the authors resort to smoothed analysis: 
%the idea is to perturb the cost matrix in order to obtain a perturbed SDP that is not in the pathological set with high probability. More 
%specifically, if $Y\in \K^{n\times k}$ is an ASOSP of the perturbed version of (P-P) with $k=\tilde{\Omega}(\sqrt{m})$ and the residues 
%$\left(\dotprod{A_i,X}-b_i\right)^2$ are bounded for $i=1,\dots,m$, then they establish that $X=YY^{*}$ is an approximate global 
%optimum of (P-SDP). One important drawback of this work is that the final result does not hold for the original SDP, but 
%for a non-equivalent penalized version of it. This is one of the points we improve here, for the case of smooth SDPs.
%
%
%
%
%

